Encoder-based Domain Tuning for Fast Personalization of Text-to-Image Models

Text-to-image personalization aims to teach a pre-trained diffusion model to reason about novel, user provided concepts, embedding them into new scenes guided by natural language prompts. However, current personalization approaches struggle with lengthy training times, high storage requirements or loss of identity. To overcome these limitations, we propose an encoder-based domain-tuning approach. Our key insight is that by underfitting on a large set of concepts from a given domain, we can improve generalization and create a model that is more amenable to quickly adding novel concepts from the same domain. Specifically, we employ two components: First, an encoder that takes as an input a single image of a target concept from a given domain, e.g. a specific face, and learns to map it into a word-embedding representing the concept. Second, a set of regularized weight-offsets for the text-to-image model that learn how to effectively ingest additional concepts. Together, these components are used to guide the learning of unseen concepts, allowing us to personalize a model using only a single image and as few as 5 training steps - accelerating personalization from dozens of minutes to seconds, while preserving quality.

==> 06-limitations.tex <==
\section{Limitations}

While our method can achieve high-fidelity personalization with short training times, it is not free of limitations. First, our encoders learn to generalize from large datasets that represent the coarse target class. As such, they are only applicable for classes where large datasets exist. In practice, this includes both faces and artistic styles which are the current primary use-cases for personalization. However, it may limit their applicability to rare, one-of-a-kind objects. In \cref{fig:cross_domain} we show the effects of trying to personalize out-of-domain images using our method. When the concepts are from nearby domains (dogs, inverted with a model trained on cats), the method can still produce high-fidelity results. For farther domains (a wooden toy) the method fails to capture concept-specific details.

A further limitation is in the need to perform inference-time tuning. While the impact on synthesis times is short, our approach does require the inference-machine to be capable of tuning a model. Moreover, as the encoder and text-to-image models must be tuned in tandem, this process requires more memory than direct fine-tuning approaches.


